CPGAN: Full-Spectrum Content-Parsing Generative Adversarial Networks for Text-to-Image Synthesis

Typical methods for text-to-image synthesis seek to design effective generative architecture to model the text-to-image mapping directly. It is fairly arduous due to the cross-modality translation. In this paper we circumvent this problem by focusing on parsing the content of both the input text and the synthesized image thoroughly to model the text-to-image consistency in the semantic level. Particularly, we design a memory structure to parse the textual content by exploring semantic correspondence between each word in the vocabulary to its various visual contexts across relevant images during text encoding. Meanwhile, the synthesized image is parsed to learn its semantics in an object-aware manner. Moreover, we customize a conditional discriminator to model the fine-grained correlations between words and image sub-regions to push for the text-image semantic alignment. Extensive experiments on COCO dataset manifest that our model advances the state-of-the-art performance significantly (from 35.69 to 52.73 in Inception Score).

==> 5_supplement_material.tex <==
\section{Details of Coarse-to-fine Generative Framework}

As described in Sec 3.1 in the paper, we adopt three cascaded generators to obtain coarse-to-fine synthesized images. At each stage, the generator $G_i$ is adopted to generate intermediate feature maps $\mathbf{C_i}$ which could be directly mapped to generated image by convolutional layers.

\begin{figure}[t]
\centering
\includegraphics[height=3.5cm]{Images/supplement.pdf}
\caption{Illustration of the coarse-to-fine framework of our CPGAN: (a) the structure of the initial generator $G_0$; (b) the structure of generators $G_1, G_2$; (c) the structure of unconditional discriminator.}
\label{fig:supplement}
\end{figure}

As shown in Figure~\ref{fig:supplement} (a), the global embedding for the whole sentence $\mathbf{s}$ concatenated with Gaussian noise $\mathbf{z}$ is processed by $G_0$, which is composed of a FC layer, a reshape layer and four cascaded upsampling layers. The obtain intermediate feature map $\mathbf{C_0}$, together with $\mathbf{H_0}$, are then fed into 
the subsequent generators $G_1$ and $G_2$, which consists of three residual blocks and a upsampling layer. 
Here $\mathbf{H_0}$ is the output of the attention model $F^{att}$ designed  to attend to the word embeddings $\mathbf{W}$ to each pixel of $\mathbf{C_0}$.
Formally, given the input word embedding $\mathbf{W} = \{\mathbf{w}_1, \mathbf{w}_2, \dots \mathbf{w}_T \}$ and the intermediate feature map $\mathbf{C_i} \in \mathbb{R}^{\hat{d} \times N_{i} \times N_{i}}$, the $\mathbf{H_i}$ is modeled as:
\begin{align}
    \mathbf{H_i} = F^{att}_i(\mathbf{W}, \mathbf{C_{i}}), \quad i=0, 1.
    \label{eqn:Fatt}
\end{align}
Herein $N_{i} \times N_{i}$ is the shape of intermediate feature map at the stage $i$ and $\mathbf{w}_t \in \mathbb{R}^{d}$ denotes the embedding for the $t$-th word.
The word embeddings are first projected into the common space of the intermediate features by a FC layer, $i.e., {\mathbf{\hat{w}}_t} = \mathbf{M}_{p}\mathbf{w}_{t}$, where $\mathbf{M}_{p} \in \mathbb{R}^{\hat{d} \times d}$.
Suppose the $(m,n)$-th intermediate feature in the feature map is denoted as $\mathbf{C_i}^{m,n} \in \mathbb{R}^{\hat{d}},m,n \in 1,2,3,...,N_{i}$.
We compute the dynamic representation of word embeddings related to the $(m,n)$-th intermediate feature by attention mechanism:
\begin{align}
\begin{split}
&b_k = \frac{\exp({(\mathbf{C_i}^{m,n})^{T} \mathbf{\hat{w}}_k})}{\sum_{p=1}^T \exp({(\mathbf{C_i}^{m,n})^{T} \mathbf{\hat{w}}_p})}, n=1, 2, \dots, T, \\
&\mathbf{H_i}^{m,n} = \sum_{k=1}^{T} b_k \mathbf{\hat{w}}_k,
\end{split}
\end{align}
where $\mathbf{H_i} \in \mathbb{R}^{\hat{d} \times N_i \times N_i}$ is the dynamic representation of word embeddings related to the intermediate feature maps $\mathbf{C_i}$.

\section{The Structure of Unconditional Discriminators}
The unconditional discriminator $D_i^{uc}$ in Sec 3.1 in the paper consists of five cascaded downsampling layers, a Reshape layer and a FC layer, as illustrated in Figure~\ref{fig:supplement} (c).

\section{DAMSM Loss}
We employ DAMSM~\cite{xu2018attngan} to construct our TISCL loss function for modeling the non-matching loss between a textual description $X$ and the corresponding synthesized image $\widetilde{I}$.
%As shown in Equation 13 in the main paper, the key difference between our TISCL and DAMSM lies in encoding mechanisms for both input text and the synthesized image .
Formally, given the final word embeddings $\mathbf{W} = \{\mathbf{w}_1, \mathbf{w}_2, \dots \mathbf{w}_T \}$ and sentence embedding $\mathbf{s}$ obtained by our text encoder in Equation 8 in the paper and the image embedding $\mathbf{V} \in \mathbb{R}^{256 \times 100}$ by our image encoder shown in Equation 9 in the paper, the TISCL is modeled as:
\begin{align}
\mathcal{L}_{\text{TISCL}} = \mathcal{L}_{\text{DAMSM}} (\mathbf{W}, \mathbf{s}, \mathbf{V}, \mathbf{f}).
\label{eqn:tiscl}
\end{align}
Here $\mathbf{f} \in \mathbb{R}^{d}$ is the image global feature extracted from the last average pooling layer of Inception-V3. 
We use $\mathbf{w}_T$ as the sentence embedding $\mathbf{s} \in \mathbb{R}^{d}$.

We first reshape $\mathbf{W}$ into matrix $\mathbf{\bar{W}} \in \mathbb{R}^{d \times T}$.
The similarity matrix for pairs of words and sub-regions is computed by:
\begin{align}
\mathbf{Sim} = (\mathbf{\bar{W}})^{T} \mathbf{V},
\end{align}
where $\mathbf{Sim}_{i,j}$ is the dot-product similarity between the $i$-th word of the sentence and the the $j$-th sub-region of the image.
We calculate the dynamic representation $\mathbf{c}_i$ for the word embedding $\mathbf{w}_i$ attending to the sub-regions of the image features by:

\begin{align}
\mathbf{\bar{Sim}}_{i,j} = \frac{\exp({\mathbf{Sim}_{i,j}) }}{\sum_{k=1}^{T} \exp({(\mathbf{Sim}_{k,j}})}, 
\end{align}

\begin{align}
\alpha_j = \frac{\exp({\gamma_1 \mathbf{\bar{Sim}}_{i,j}) }}{\sum_{k=1}^{100} \exp({(\gamma_1 \mathbf{\bar{Sim}}_{i,k}})}, 
\end{align}

\begin{align}
\mathbf{c}_i = \sum_{j=1}^{100} \alpha_j \mathbf{V}[:,j],
\end{align}
where $\gamma_1$ is a factor that determines how much attention is paid to features of its relevant sub-regions when computing
the region-context vector for a word.
Finally, we define the semantic consistency between each word of input text and different sub-region of the image using the cosine similarity, $i.e., R(\mathbf{c}_i,\mathbf{w}_i)=(\mathbf{c}_i^{T} \mathbf{w}_i)/(||\mathbf{c}_i||||\mathbf{w}_i||)$.
The image-text matching score between the entire image $\mathbf{I}$ and the whole sentence description $\textbf{D}$ is define as:
\begin{align}
R(\mathbf{I},\mathbf{D}) = \log(\sum_{i=1}^{T} \exp(\gamma_2 R(\mathbf{c}_i,\mathbf{w}_i)))^{1/\gamma_2},
\end{align}
where $\gamma_2$ is a factor that determines how much to magnify the importance of the most relevant word-to-region-context pair.

In a mini-batch of iteration, the posterior probability of sentence $\mathbf{D}_i$ matching with the corresponding image $\mathbf{I}_i$ is obtained by:
\begin{align}
P(\mathbf{D}_i|\mathbf{I}_i) = \frac{\exp(R(\gamma_3\mathbf{I}_i,\mathbf{D}_i))}{\sum_{j=1}^{M} \exp( R(\gamma_3\mathbf{I}_i,\mathbf{D}_j))},
\end{align}
where $\gamma_3$ is a smoothing factor determined by experiments. $M$ is batch size.
Then the word-level loss function of the positive image-sentence pair in a mini-batch is define as:
\begin{align}
	\mathcal{L}^{w} = -\sum_{i=1}^{M}\log P(\mathbf{D}_i|\mathbf{I}_i) + \log P(\mathbf{I}_i|\mathbf{D}_i)
\end{align}
For the sentence embedding $\mathbf{s}$ and the image global feature  $\mathbf{f}$, we define the image-text matching score by:
\begin{align}
\hat{R}(\mathbf{I},\mathbf{D}) = (\mathbf{f}^\top \mathbf{s})/ (||\mathbf{f}^\top||||\mathbf{s}||).
\end{align}
The sentence-level loss $\mathcal{L}^{s}$ is modeled as:
\begin{align}
\hat{P}(\mathbf{D}_i|\mathbf{I}_i) = \frac{\exp(\hat{R}(\gamma_3\mathbf{I}_i,\mathbf{D}_i))}{\sum_{j=1}^{M} \exp( \hat{R}(\gamma_3\mathbf{I}_i,\mathbf{D}_j))} 
\end{align}
\begin{align}
\mathcal{L}^{s} = -\sum_{i=1}^{M}\log \hat{P}(\mathbf{D}_i|\mathbf{I}_i) + \log \hat{P}(\mathbf{I}_i|\mathbf{D}_i)
\end{align}
Finally, the DAMSM loss is define as:
\begin{align}
\mathcal{L}_{DAMSM} = \mathcal{L}^{w} + \mathcal{L}^{s}
\end{align}



